Multimodal embodiment-aware navigation transformer

Goal-conditioned navigation models for ground robots trained using supervised learning show promising zero-shot transfer, but their collision-avoidance capability nevertheless degrades under distribution shift, i.e. environmental, robot or sensor configuration changes. We propose ViLiNT a multimodal, attention-based policy for goal navigation, trained on heterogeneous data from multiple platforms and environments, which improves robustness with two key features. First, we fuse RGB images, 3D LiDAR point clouds, a goal embedding and a robot's embodiment descriptor with a transformer architecture to capture complementary geometry and appearance cues. The transformer's output is used to condition a diffusion model that generates navigable trajectories. Second, using automatically generated offline labels, we train a path clearance prediction head for scoring and ranking trajectories produced by the diffusion model. The diffusion conditioning as well as the trajectory ranking head depend on a robot's embodiment token that allows our model to generate and select trajectories with respect to the robot's dimensions. Across three simulated environments, ViLiNT improves Success Rate on average by 166\% over equivalent state-of-the-art vision-only baseline (NoMaD). This increase in performance is confirmed through real-world deployments of a rover navigating in obstacle fields. These results highlight that combining multimodal fusion with our collision prediction mechanism leads to improved off-road navigation robustness.

==> figures/architecture.tex <==
\begin{figure*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  font=\footnotesize,
  node distance=4mm and 7mm,
  arrow/.style={-Latex, line width=0.7pt},
  data/.style={draw, rounded corners=2pt, align=center, inner sep=3pt, fill=blue!6},
  op/.style={draw, rounded corners=2pt, line width=0.7pt, align=center, inner sep=4pt, fill=orange!10},
  model/.style={draw, rounded corners=2pt, line width=0.8pt, align=center, inner sep=4pt, fill=teal!10},
  loss/.style={draw, diamond, aspect=2, line width=0.7pt, align=center, inner sep=1.2pt, fill=red!8}
]

% Inputs
\node[data] (rgb) {RGB $\{\mathbf{I}_{t-k:t}\}$};
\node[data, below=of rgb] (lidar) {LiDAR $\mathbf{L}_t$};
\node[data, below=of lidar] (goal) {Goal $\mathbf{g}$};
\node[data, below=of goal] (state) {State $\mathbf{x}_t$};

% Encoders + tokenization + type/time
\node[op, right=10mm of rgb, yshift=-6mm, minimum width=28mm] (enc)
{Encoders \& tokenizers\\\footnotesize + type/time embeds};

\draw[arrow] (rgb.east) -- (enc.west);
\draw[arrow] (lidar.east) -- (enc.west);
\draw[arrow] (goal.east) -- (enc.west);
\draw[arrow] (state.east) -- (enc.west);

% Transformer -> context
\node[model, right=8mm of enc, minimum width=26mm] (xfmr) {Cross-modal Transformer};
\node[data, right=7mm of xfmr, minimum width=22mm] (ctx) {Context $\mathbf{C}\in\mathbb{R}^{N\times d}$};
\draw[arrow] (enc) -- node[above]{\scriptsize tokens} (xfmr);
\draw[arrow] (xfmr) -- (ctx);

% Diffusion branch
\node[model, right=9mm of ctx, yshift=8mm, minimum width=28mm] (diff) {Goal-cond. diffusion head $\epsilon_\theta$};
\draw[arrow] (ctx) -- (diff);
\node[data, above left=5mm and -1mm of diff] (gtY) {GT traj $\mathbf{Y}$};
\node[data, above=5mm of diff, xshift=10mm] (noise) {$\boldsymbol\epsilon,\ t$};
\node[op, right=6mm of noise, minimum width=28mm] (forw)
{$\tilde{\mathbf{Y}}=\sqrt{\bar\alpha_t}\mathbf{Y}+\sqrt{1-\bar\alpha_t}\boldsymbol\epsilon$};
\draw[arrow] (gtY) |- (forw);
\draw[arrow] (noise) -- (forw);
\draw[arrow] (forw) |- (diff.west);

\node[data, right=6mm of diff] (epshat) {$\hat{\boldsymbol\epsilon}$};
\node[loss, right=5mm of epshat] (ldiff) {$\mathcal{L}_{\text{diff}}$};
\draw[arrow] (diff) -- (epshat);
\draw[arrow] (epshat) -- (ldiff);

% Optional waypoint aux
\node[op, below=5mm of diff, minimum width=26mm] (denoise) {Denoise (teacher-forcing)};
\node[data, right=5mm of denoise] (yhat) {$\hat{\mathbf{Y}}$};
\node[loss, right=5mm of yhat] (lwp) {$\mathcal{L}_{\text{wp}}$};
\draw[arrow] (ctx) |- (denoise);
\draw[arrow] (denoise) -- (yhat);
\draw[arrow] (gtY) |- (lwp);
\draw[arrow] (yhat) -- (lwp);

% Collision branch
\node[model, below=12mm of ctx, minimum width=28mm] (coll) {Collision head $s_\phi(\mathbf{C},\mathbf{Y},w)$};
\draw[arrow] (ctx) -- (coll);
\node[data, below left=4mm and 2mm of coll] (ysrc) {$\mathbf{Y}\in\{\text{GT},\ \hat{\mathbf{Y}}\}$};
\node[data, below right=4mm and 2mm of coll] (w) {Width $w\sim\mathcal{W}$};
\draw[arrow] (ysrc) -- (coll);
\draw[arrow] (w) -- (coll);

\node[op, below=5mm of ysrc, minimum width=46mm, fill=violet!12] (ss)
{Self-supervision from LiDAR:\\min-corridor width / TTC};
\node[data, right=5mm of ss] (label) {Label $y_w$};
\draw[arrow] (lidar) |- (ss);
\draw[arrow] (ss) -- (label);

\node[loss, right=6mm of coll] (lbce) {$\mathcal{L}_{\text{bce}}$ / $\mathcal{L}_{\text{rank}}$};
\draw[arrow] (coll) -- (lbce);
\draw[arrow] (label) |- (lbce);

% Total loss (compact)
\node[loss, right=6mm of ldiff, yshift=-6mm, text width=48mm, inner sep=2pt] (ltotal)
{$\lambda_{\text{diff}}\mathcal{L}_{\text{diff}}+\lambda_{\text{wp}}\mathcal{L}_{\text{wp}}+\lambda_{\text{bce}}\mathcal{L}_{\text{bce}}+\lambda_{\text{rank}}\mathcal{L}_{\text{rank}}$};
\draw[arrow] (ldiff) -- (ltotal);
\draw[arrow] (lwp) -- (ltotal);
\draw[arrow] (lbce) -- (ltotal);

% Tiny legend
\node[draw, rounded corners=2pt, inner sep=2pt, below=6mm of state, align=left, fill=white] (leg) {%
\begin{tabular}{@{}ll@{}}
\tikz{\node[data, minimum width=6mm, minimum height=2.5mm]{};} & Data \\
\tikz{\node[op, minimum width=6mm, minimum height=2.5mm]{};} & Encoder/Op \\
\tikz{\node[model, minimum width=6mm, minimum height=2.5mm]{};} & Model head \\
\tikz{\node[loss, minimum width=6mm, minimum height=2.5mm]{};} & Loss \\
\end{tabular}};
\end{tikzpicture}
}%
\caption{Training/learning: multimodal tokenization $\to$ cross-modal Transformer context, goal-conditioned diffusion noise-prediction (with optional waypoint regression), and self-supervised collision head using LiDAR-derived labels (min-corridor width / TTC).}
\label{fig:train_full}
\end{figure*}

\begin{figure*}[!b]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  font=\footnotesize,
  node distance=4mm and 7mm,
  arrow/.style={-Latex, line width=0.7pt},
  data/.style={draw, rounded corners=2pt, align=center, inner sep=3pt, fill=blue!6},
  op/.style={draw, rounded corners=2pt, line width=0.7pt, align=center, inner sep=4pt, fill=orange!10},
  model/.style={draw, rounded corners=2pt, line width=0.8pt, align=center, inner sep=4pt, fill=teal!10}
]

% Inputs
\node[data] (rgb2) {RGB $\{\mathbf{I}_{t-k:t}\}$};
\node[data, below=of rgb2] (lidar2) {LiDAR $\mathbf{L}_t$};
\node[data, below=of lidar2] (goal2) {Goal $\mathbf{g}$};
\node[data, below=of goal2] (state2) {State $\mathbf{x}_t$};

% Encoders + Transformer -> context
\node[op, right=10mm of rgb2, yshift=-6mm, minimum width=28mm] (enc2) {Encoders \& tokenizers\\\footnotesize + type/time embeds};
\node[model, right=8mm of enc2, minimum width=26mm] (xfmr2) {Cross-modal Transformer};
\node[data, right=7mm of xfmr2] (c2) {Context $\mathbf{C}$};
\draw[arrow] (rgb2) -- (enc2);
\draw[arrow] (lidar2) -- (enc2);
\draw[arrow] (goal2) -- (enc2);
\draw[arrow] (state2) -- (enc2);
\draw[arrow] (enc2) -- (xfmr2);
\draw[arrow] (xfmr2) -- (c2);

% Diffusion sampler
\node[model, right=8mm of c2, minimum width=28mm] (sampler)
{Diffusion sampler\\$N$ candidates $\{\mathbf{Y}_i\}$};
\draw[arrow] (c2) -- (sampler);

% Collision scoring
\node[model, right=8mm of sampler, minimum width=28mm] (score)
{Collision head\\$s_\phi(\mathbf{C},\mathbf{Y}_i,w)$};
\node[data, below=of score] (w2) {Width $w$};
\draw[arrow] (sampler) -- (score);
\draw[arrow] (w2) -- (score);

% Selection
\node[op, right=8mm of score, align=left, minimum width=34mm, fill=green!12] (select)
{Select $\displaystyle \arg\min_i\ \lambda_{\text{goal}}\,d(\mathbf{Y}_i,\mathbf{g})+\lambda_{\text{risk}}\,s_\phi$};

% Controller output
\node[data, right=8mm of select, align=center, fill=blue!6] (ctrl)
{First waypoint(s)\\$\rightarrow$ PX4 / controller};

\draw[arrow] (score) -- (select);
\draw[arrow] (select) -- (ctrl);

\end{tikzpicture}
}%
\caption{Inference/deployment: sample $N$ candidate trajectories from the diffusion policy, score collision risk per candidate and width, then choose the lowest-cost plan and send the first waypoint(s) to the controller.}
\label{fig:infer_full}
\end{figure*}
